Automatic Digitization and Orientation of Scanned Mesh Data for Floor Plan and 3D Model Generation

This paper describes a novel approach for generating accurate floor plans and 3D models of building interiors using scanned mesh data. Unlike previous methods, which begin with a high resolution point cloud from a laser range-finder, our approach begins with triangle mesh data, as from a Microsoft HoloLens. It generates two types of floor plans, a "pen-and-ink" style that preserves details and a drafting-style that reduces clutter. It processes the 3D model for use in applications by aligning it with coordinate axes, annotating important objects, dividing it into stories, and removing the ceiling. Its performance is evaluated on commercial and residential buildings, with experiments to assess quality and dimensional accuracy. Our approach demonstrates promising potential for automatic digitization and orientation of scanned mesh data, enabling floor plan and 3D model generation in various applications such as navigation, interior design, furniture placement, facilities management, building construction, and HVAC design.

==> 4a-results.tex <==
%=======================================
\section{Results and Discussion}~\label{sec:res}
%=======================================

\subsection{Floor plans}
Add blownup version furniture
\subsection{Multi-level slicing}


% To evaluate our overall approach, we run our algorithm on two different scene shown in Figure~\ref{fig:Benchmark1} and Figure~\ref{fig:Benchmark2}. In both the scene, the switching cost ${S_c}$ is kept same while ${M_c}$ have been changed to obtain path of different length and cost.  Table\~\ref{tab:analysis} shows analysis for the two scenes. 

% In scene 1, the clearance used are 8, 11 and 14 units. If the corridor with a particular clearance value is chosen during path extraction, the formation passing through that corridor will have size no bigger than the clearance value. It can be seen in top row of Figure~\ref{fig:Benchmark1}, the group of agent forming a circular formation reduces in size when passing through the narrow corridor.  


% we have investigated the use of our algorithm in three different types of environments. In all the chosen environment, the switching cost ${S_c}$ and movement cost ${M_c}$ are varied to compute the length of shortest path ${{PL}}$ and time taken by the group to reach goal position from start position ${TT}$. Also, number of SPM ${NS}$
\begin{table}[h]
\caption{Analysis} %title of the table
\centering % centering table
\begin{tabular}{c rrr} % creating eight columns
\hline\hline %inserting double-line
Scenarios & $T_Or$ & $T_sl$  &  $T_fp$\\ \hline
Scene 1 &  &  &   \\ 
Scene 2 &  &  &   \\ 
Scene 3 &  &  &   \\ 
\hline % inserts single-line
\end{tabular}
\label{tab:analysis}
\end{table}


% \begin{figure}[h]
%   \centering
%   \label{fig:Benchmark1}
%   \includegraphics[width=\columnwidth]{figures/Benchmark1.png}
%   \caption{Scene 1: From left to right, Top images shows animation sequence at 475s, 1190s and 1718s.Middle images shows animation sequence at 475s, 1190s and 3095s, Bottom images shows animation sequence at 475s, 1190s and 2663s. The time step and simulations per frame update used for this benchmark are 0.08 secs and 20 respectively.}
% \end{figure}
% \begin{figure}[h]
%   \centering
%   \label{fig:Benchmark2}
%   \includegraphics[width=\columnwidth]{figures/Benchmark2.png}
%   \caption{Scene 2: From left to right, Top images shows animation sequence at 64s, 190s and 261s.Middle images shows animation sequence at 64s, 190s and 244s, Bottom images shows animation sequence at 64s, 190s and 309s. The time step and simulations per frame update used for this benchmark are 0.08 secs and 20 respectively.}
% \end{figure}


% %=FIGURE==================================
% %\begin{figure*}[th]
% %  \centering
% %  \includegraphics[width=0.32\textwidth]{figures/cf1-reduced.png} 
% %  \includegraphics[width=0.31\textwidth]{figures/cf22.png}
% %  \caption{\label{fig:strategies}
% %   The etc
% %  }
% %\end{figure*}
% %=========================================


% %=FIGURE==================================
% %\begin{figure}[th]
% %  \centering
% %  \includegraphics[width=0.43\columnwidth]{figures/user4.jpg} 
% %  \includegraphics[width=0.52\columnwidth]{figures/user5.jpg}
% %  \caption{\label{fig:exusers}
% %  Two participants in our user study.
% %           }
% %\end{figure}
% %=========================================


==> 6-supplementarymaterial.tex <==
\newpage
\clearpage
\section*{Supplemental Materials}
Due to the space limitation in the manuscript, we include additional algorithms and figures in this supplemental section.

\subsection*{Orienting the floor using a bounding box}
It is often the case that one story of a building will be larger horizontally than vertically, that the ceiling will be at a constant altitude, and that the floor will be at a constant altitude. In this case, a simple bounding box method is enough to orient the mesh $\mathcal{M}$ so that its floor is level (at a constant y value). 

% In this case, we can proceed as follows:

\vspace{-0.3cm}
\begin{algorithm}
\caption{Orienting the floor using the bounding box method}
\begin{algorithmic}[1]
  \State $\mathcal{BB}~\gets$ \textit{ComputeBoundingBox}$(\mathcal{M})$;
  \State $\vec{g_{m}}~\gets$ \textit{ComputeModelGravityFromBox}$(\mathcal{BB})$;
  \State $\vec{g_{t}}~\gets$ -$\vec{y}$;
  \State $\theta~\gets \arccos(\vec{g_{t}}$ . $\vec{g_{m}})$;
  \State $\mathcal{Y}~\gets$ $\vec{g_{t}}$ x $\vec{g_{m}}$;
  \State $\mathcal{M}$~$\gets$ $\textit{rotateMesh}$ $(\theta, \mathcal{Y})$;
\end{algorithmic}
\label{alg:BBMethod}
\end{algorithm}
\vspace{-0.3cm}

To orient the mesh $\mathcal{M}$ based on its bounding box, first, a tightly fitting bounding box $\mathcal{BB}$ is computed. The vertical dimension of the bounding box is assumed to be the minimum dimension. Then, the surface normal of the top face of this bounding box, pointing towards the interior, is calculated to obtain an approximation of the true gravity direction $\vec{g_{m}}$. The angle $\theta$ is computed using the dot product of $\vec{g_{t}}$ and $\vec{g_{m}}$ followed by applying the arccosine function. The axis of rotation $\mathcal{Y}$ is computed by taking the cross product of those vectors. The mesh is then rotated by $\theta$ along the $\mathcal{Y}$ axis, resulting in a horizontal floor. For a more detailed formal description of the bounding box method, please refer to Algorithm~\ref{alg:BBMethod}.


\subsection*{Opacity and Slicing Experiment}
To determine appropriate opacity and slicing, we first varied the opacity across values of 0.1, 0.3, 0.5, 0.7, and 0.9 while keeping the number of slices constant. The results of our opacity test, as shown in Figure~\ref{fig:OpacityTest}, indicate that an opacity of 0.5 yields a satisfactory floor plan. Next, we tested the effect of increasing or decreasing the number of slices used to create a pen-and-ink style floor plan. As we increase the number of slices, more details such as furniture shapes and tabletops become visible. Conversely, reducing the number of slices produces a lighter, less cluttered floor plan. Figure~\ref{fig:slicingTest} illustrates the results of our slicing test. We determined that generating a floor plan with 100 slices balances detail and clutter reduction well, but depending on the use case, other values may be more desirable.

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{figures/100Slices_withMultipleOpacity.png}
  \centering
  \caption{Pen-and-ink style floor plans with opacity equal to 0.1, 0.3, 0.5, 0.7 and 0.9 from left to right.}
  \label{fig:OpacityTest}
\end{figure*}
\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{figures/SlicingTestWith0.5Transparency.png}
  \centering
  \caption{Pen-and-ink style floor plans with slice count equal to 50, 75, 100, and, 150 from left to right.}
  \label{fig:slicingTest}
\end{figure*}

\subsection*{Additional results} 
In this section, we present the results obtained from various stages of our approach that led to the computation of floor plans and extraction of flat walls. The computational time for each major step involved in the computation of floor plans and extraction of flat walls is provided in Table~\ref{tab:more_analysis1} and Table~\ref{tab:more_analysis2} for single-story and multi-story buildings, respectively. Models 1, 2, and 3 represent single-story buildings, while models 4 and 5 represent multi-story buildings.

\begin{table}[!ht]
\caption{Computational Times(in Seconds): $T_o$, $T_p$, $T_{D_{fp}}$ are the time for orienting mesh, finding planar walls and, computing drafting style floor plan in seconds for a single story building} %title of the table
\centering % centering table
\begin{tabular}{c | rrr} % creating three columns
\hline\hline %inserting double-line
Model  & $T_o$ & $T_p$ &  $T_{D_{fp}}$\\ \hline
1  & 4.63 & 15.17  &  0.51\\
2  &  1.26 & 10.62 & 0.21  \\ 
3  & 42.77  & 174.19 &  1.14  \\ 
\hline % inserts single-line
\end{tabular}
\label{tab:more_analysis1}
\end{table}


\begin{table}[!ht]
\caption{Computational Times(in Seconds): $T_o$, $T_p$, $T_{pr}$ are the total time for orienting mesh of entire building, finding planar walls, and computing drafting style floor plan in seconds for each level of multistory building} %title of the table
\centering % centering table
\begin{tabular}{c | c | rrr} % creating three columns
\hline\hline %inserting double-line
Model &  level &$T_o$ & $T_p$ &  $T_{D_{fp}}$\\ \hline
4  & 0 & 23.92 & 43.6 &  0.41\\
4  & 1 &   & 39.5  &  0.43\\ \hline
5  & 0 & 41.6 &41.70 & 0.62  \\ 
5  & 1 & & 54.44 & 1.24  \\ 
5  & 2 & & 37.97 & 0.99  \\ 
\hline % inserts single-line
\end{tabular}
\label{tab:more_analysis2}
\end{table}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{figures/ornl_rotation_and_ceiling_removal.png}
  \centering
  \caption{ Model 1: (a) Scanned mesh data of a building. (b) Oriented mesh using Spherical K-means. (c,d) Building with ceiling and floor removed respectively. (e) Histogram used for ceiling and floor detection }
  \label{fig:ornl_model1}
\end{figure*}
\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/ornl_FP_walls.png}
  \centering
  \caption{Model 1: (a) Cluster obtained using DBSCAN (b) Flat Walls (c) Flat walls with the building model. (d,e) Drafting and Pen-and-Ink style floor plan respectively.}
  \label{fig:ornl_model2}
\end{figure*}


\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/MeshDefault_ISG_rotation_and_ceiling_removal.png}
  \centering
  \caption{Model 2: (a) Scanned mesh data of a building. (b) Oriented mesh using Spherical K-means. (c,d) Building with ceiling and floor removed respectively. (e) Histogram used for ceiling and floor detection }
  \label{fig:model_isg1}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/MeshDefault_ISG_FP_walls.png}
  \centering
  \caption{Model 2: (a) Cluster obtained using DBSCAN (b) Flat Walls (c) Flat walls with the building model. (d,e) Drafting and Pen-and-Ink style floor plan respectively.}
  \label{fig:model_isg2}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/Mesh20211021194212_rotation_and_ceiling_removal.png}
  \centering
  \caption{Model 3: (a) Scanned mesh data of a building. (b) Oriented mesh using Spherical K-means. (c,d) Building with ceiling and floor removed respectively. (e) Histogram used for ceiling and floor detection }
  \label{fig:Mesh20211021194212_1}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/Mesh20211021194212_FP_walls.png}
  \centering
  \caption{Model 3: (a) Cluster obtained using DBSCAN (b) Flat Walls (c) Flat walls with the building model. (d,e) Drafting and Pen-and-Ink style floor plan respectively.}
  \label{fig:Mesh20211021194212_2}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/LesHouse_level1_level2.png}
  \centering
  \caption{Model 4: (a) Scanned mesh data of a two-story building. (b) Oriented mesh using Spherical K-means. (c,d) level 0 and level 1 of the two-story building after partition. (e) Histogram used for partitioning the building }
  \label{fig:LesHouse_level1_level2_1}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/LesHouse_level1_level2_FP.png}
  \centering
  \caption{Model 4: Left to right: Show clusters, flat walls, flat walls with building, drafting style  and pen-and-ink style floor plan for level 0 (top row) and level 1 (bottom row). }
  \label{fig:LesHouse_level1_level2_2}
\end{figure*}


\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/matterport_level1_level2_level3.png}
  \centering
  \caption{Model 5: (a) Scanned mesh data of a three-story building. (b) Oriented mesh using Spherical K-means. (c,d,e) level 0, level 1 and level 2 of the three-story building after partition. (f) Histogram used for partitioning the building }
  \label{fig:matterport_level012_1}
\end{figure*}

\begin{figure*}[!ht]
  \includegraphics[width=\linewidth]{cgi2018_latex/figures/matterport_level1_level2_level3_FP.png}
  \centering
  \caption{Model 5: Left to right: Show clusters, flat walls, flat walls with building, drafting style  and pen-and-ink style floor plan for level 0 (top row) level 1 (middle row) and level 2 (bottom row). }
  \label{fig:matterport_level012_2}
\end{figure*}
